LLM Value Functions for Credit Assignment in Agentic RL

Reinforcement learning (RL) for large language model (LLM) agents remains challenging in long-horizon tasks with sparse outcome rewards, where assigning credit to individual actions is difficult. Methods such as GRPO assign the same trajectory-level advantage to all actions, while critic-based methods require learning an additional value function that can be costly and unstable. We introduce LLM Value Function RL (LVRL), which uses the pretrained knowledge and in-context learning ability of an LLM to estimate policy-aware state values without finetuning a separate critic. LVRL conditions the value model on group context and calibrates its predictions using known values at the initial and terminal states, enabling step-level credit assignment from estimated value differences. We further extend this idea to learning from an expert policy through on-policy distillation (OPD), introducing LLM Value Function OPD (LVOPD), which focuses teacher supervision on actions associated with decreases in estimated value. We evaluate our approach across diverse agentic benchmarks: AppWorld, BabyAI, and SWE-bench Verified. Across policy scales (4B to 32B), LVRL consistently and substantially outperforms both GRPO and PPO. On AppWorld and SWE-bench Verified, LVRL yields absolute improvements of up to 13.6 and 8.6 percentage points over GRPO. Notably, on tasks requiring extended exploration like BabyAI, LVRL bridges the gap from total failure to 75.0% success. Furthermore, LVOPD yields consistent improvements over standard distillation baselines on AppWorld. Finally, Monte-Carlo analysis confirms that our frozen critic accurately identifies semantic pitfalls and recoveries, proving that LVRL extracts robust, policy-aware step-level credit from sparse terminal outcomes.

==> figs/figure.tex <==
% =====================================================================
%  PREAMBLE  (main.tex)
% =====================================================================
\usepackage{tikz}
\usepackage{xcolor}

\definecolor{bWall}{HTML}{3D4451}
\definecolor{bFloor}{HTML}{F4F4F2}
\definecolor{bDoor}{HTML}{E0A106}
\definecolor{bObj}{HTML}{B9BDC4}
\definecolor{bTarget}{HTML}{C0392B}
\definecolor{bPath}{HTML}{2E86AB}
\definecolor{bAgent}{HTML}{1E8449}

\newlength{\bcell}\setlength{\bcell}{6.4pt}   % 19 cells ~ 1.69in per panel

\tikzset{
  bwall/.style       = {fill=bWall},
  bfloor/.style      = {fill=bFloor},
  bdoor/.style       = {fill=bDoor},
  bobj/.style        = {fill=bObj},
  btarget/.style     = {fill=bTarget},
  btargetring/.style = {draw=bTarget,line width=0.5pt},
  bagent/.style      = {fill=bAgent},
  bpathcase/.style   = {draw=white,line width=3.2pt,
                        line cap=round,line join=round},
  bpath/.style       = {draw=bPath,line width=1.5pt,opacity=0.85,
                        line cap=round,line join=round},
}

% =====================================================================
%  FIGURE
% =====================================================================
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.32\linewidth}\centering
  {\footnotesize (a) ID, door distance 1}\\[3pt]
  \input{figs/maze_a}\\[3pt]
  {\scriptsize \emph{pick up the blue ball} --- 15 actions}
\end{minipage}\hfill
\begin{minipage}[t]{0.32\linewidth}\centering
  {\footnotesize (b) ID, door distance 3}\\[3pt]
  \input{figs/maze_b}\\[3pt]
  {\scriptsize \emph{pick up the green box} --- 35 actions}
\end{minipage}\hfill
\begin{minipage}[t]{0.32\linewidth}\centering
  {\footnotesize (c) OOD, door distance 5}\\[3pt]
  \input{figs/maze_c}\\[3pt]
  {\scriptsize \emph{pick up the purple key} --- 50 actions}
\end{minipage}

\vspace{4pt}
{\footnotesize
\tikz[baseline=-0.5ex]\fill[bAgent] (0,-0.06) -- (0.18,0.06) -- (0,0.18) -- cycle;\,agent \quad
\tikz[baseline=-0.5ex]{\fill[bTarget] (0,0.06) circle (0.06); \draw[bTarget,line width=0.4pt] (0,0.06) circle (0.10);}\,target \quad
\tikz[baseline=-0.5ex]\fill[bObj] (0,0.06) circle (0.055);\,distractor \quad
\tikz[baseline=-0.5ex]\fill[bDoor] (0,-0.02) rectangle (0.16,0.14);\,closed door \quad
\tikz[baseline=-0.5ex]\draw[bPath,line width=1.2pt] (0,0.06) -- (0.3,0.06);\,shortest path}

\caption{
Representative BabyAI evaluation layouts at increasing door distance.
The blue line is the shortest collision-free path from the agent to a cell adjacent to the target; the action count below each panel additionally includes turns, door toggles, and the final pickup.
The path crosses one, three, and five doors respectively, which is what door distance measures.
Every layout holds the same inventory of $18$ objects --- three types (ball, box, key) crossed with six colors, one of each --- so the instruction names exactly one object and distractor identities carry no information; only the spatial arrangement and the choice of target vary.
All doors start closed and are never locked.
The agent never observes this map: it receives a textual egocentric description (Figure~\ref{fig:babyai-traj}).
}
\label{fig:babyai-mazes}
\end{figure}


==> tables/ablation.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}

\begin{minipage}[t]{0.48\linewidth}
\vspace{0pt}
\centering
\caption{Critic ablation on AppWorld.}
\label{tab:ablation_critic}

\begin{tabular}{@{}lc@{}}
\toprule
LLM critic & Qwen3-4B \\
\midrule
Qwen3-235B
& \meanstd{9.8}{2.3} \\

GLM-5.2
& \meanstd{23.3}{6.3} \\

Claude-Opus-4.6
& \bestmeanstd{24.3}{1.7} \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
\vspace{0pt}
\centering
\caption{Design ablation on AppWorld.}
\label{tab:ablation_design_choice}

\begin{tabular}{@{}lc@{}}
\toprule
Method & Qwen3-8B \\
\midrule
\rule[-0.66\normalbaselineskip]{0pt}{1.8\normalbaselineskip}%
\methodrl{}
& \bestmeanstd{26.3}{0.5} \\

\rule[-0.66\normalbaselineskip]{0pt}{1.8\normalbaselineskip}%
\methodrl{} w/o FS, $V(0)$
& \meanstd{22.1}{0.5} \\
\bottomrule
\end{tabular}
\end{minipage}

\end{table}

==> tables/opd_results.tex <==
\begin{table}[t]
\centering
\caption{
Evaluation performance under on-policy distillation.
}
\label{tab:main-opd}

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1} 
\resizebox{0.35\textwidth}{!}{
\begin{tabular}{@{}lcc@{}}
\toprule
& \multicolumn{2}{c}{AppWorld}
% & \multicolumn{2}{c}{BabyAI} \\
\\
\cmidrule(lr){2-3}
% \cmidrule(lr){4-5}
Method
& Qwen3-4B
& Qwen3-8B
% & Qwen3-4B
% & Qwen3-8B \\
\\
\midrule
Base
& \meanstd{4.2}{0.4}
& \meanstd{10.9}{1.0}
% & \meanstd{0.0}{0.0}\,/\,\meanstd{0.0}{0.0}
% & \bestmeanstd{0.7}{0.0}\,/\,\meanstd{0.0}{0.0} \\
\\
\midrule
+OPD
& \meanstd{17.0}{0.3}
& \meanstd{22.2}{0.7}
% & \meanstd{0.5}{0.1}\,/\,\meanstd{0.0}{0.0}
% & \meanstd{0.6}{0.3}\,/\,\meanstd{0.0}{0.0} \\
\\
+Trajectory-gated
& \meanstd{19.2}{1.0}
& \meanstd{21.2}{1.0}
% & \meanstd{0.4}{0.2}\,/\,\meanstd{0.0}{0.0}
% & \meanstd{0.3}{0.3}\,/\,\meanstd{0.0}{0.0} \\
\\
+\methodopd{} (ours)
& \bestmeanstd{20.2}{1.8}
& \bestmeanstd{23.3}{1.6}
% & \bestmeanstd{0.7}{0.2}\,/\,\meanstd{0.0}{0.0}
% & \meanstd{0.4}{0.1}\,/\,\meanstd{0.0}{0.0} \\
\\
\bottomrule
\end{tabular}
}
\end{table}



==> tables/teacher_ablation.tex <==
% \begin{table*}[t]
% \centering
% \caption{
% Evaluation performance for three environments.
% BabyAI entries report ID/OOD success rates.
% Bold indicates the best result for each environment and policy size.
% }
% \label{tab:ablation_critic}
% \small
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{lc}
% \toprule
% Teacher
% & Qwen3-4B 
% \\
% \midrule
% Qwen3-235B
% & $9.8\pm2.3$
% \\
% GLM-5.2
% & $23.3\pm6.3$
% \\
% Claude-Opus-4.6
% & $\mathbf{24.3\pm1.7}$
% \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{wraptable}{r}{0.3\textwidth}
\vspace{-\intextsep}
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{5pt}
\caption{Ablation of the different frozen LLM value critic on AppWorld.}
\label{tab:ablation_critic}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lc@{}}
\toprule
LLM critic & Qwen3-4B \\
\midrule
Qwen3-235B & \meanstd{9.8}{2.3} \\
GLM-5.2 & \meanstd{22.3}{4.1} \\
Claude Opus 4.6 & \bestmeanstd{24.3}{1.7} \\
\bottomrule
\end{tabular}
\end{wraptable}



==> tables/value_pred_ablation.tex <==
% \begin{table*}[t]
% \centering
% \caption{
% Evaluation performance for three environments.
% BabyAI entries report ID/OOD success rates.
% Bold indicates the best result for each environment and policy size.
% }
% \label{tab:ablation_design_choice}
% \small
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{lc}
% \toprule
% Method
% & Qwen3-8B
% \\
% \midrule
% \methodrl
% & $\mathbf{26.3\pm0.5}$
% \\
% \methodrl w/o FS, V(0)
% & $22.1\pm0.5$
% \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{wraptable}{r}{0.36\textwidth}
\vspace{-\intextsep}
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{5pt}
\caption{Ablation of in-context calibration for the frozen LLM value critic on AppWorld.}
\label{tab:ablation_design_choice}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lc@{}}
\toprule
Method & Qwen3-8B \\
\midrule
GRPO & \meanstd{19.8}{3.8} \\
\methodrl & \bestmeanstd{26.3}{0.5} \\
\methodrl w/o FS, $V(0)$ & \meanstd{22.1}{0.5} \\
\bottomrule
\end{tabular}
\end{wraptable}

